Certifiable Black-Box Attacks with Randomized Adversarial Examples: Breaking Defenses with Provable Confidence

Black-box adversarial attacks have demonstrated strong potential to compromise machine learning models by iteratively querying the target model or leveraging transferability from a local surrogate model. Recently, such attacks can be effectively mitigated by state-of-the-art (SOTA) defenses, e.g., detection via the pattern of sequential queries, or injecting noise into the model. To our best knowledge, we take the first step to study a new paradigm of black-box attacks with provable guarantees -- certifiable black-box attacks that can guarantee the attack success probability (ASP) of adversarial examples before querying over the target model. This new black-box attack unveils significant vulnerabilities of machine learning models, compared to traditional empirical black-box attacks, e.g., breaking strong SOTA defenses with provable confidence, constructing a space of (infinite) adversarial examples with high ASP, and the ASP of the generated adversarial examples is theoretically guaranteed without verification/queries over the target model. Specifically, we establish a novel theoretical foundation for ensuring the ASP of the black-box attack with randomized adversarial examples (AEs). Then, we propose several novel techniques to craft the randomized AEs while reducing the perturbation size for better imperceptibility. Finally, we have comprehensively evaluated the certifiable black-box attacks on the CIFAR10/100, ImageNet, and LibriSpeech datasets, while benchmarking with 16 SOTA black-box attacks, against various SOTA defenses in the domains of computer vision and speech recognition. Both theoretical and experimental results have validated the significance of the proposed attack. The code and all the benchmarks are available at \url{https://github.com/datasec-lab/CertifiedAttack}.

==> Discussion.tex <==

\section{Discussions}
\label{sec:Discussion}

\vspace{0.05in}

\noindent\textbf{Extension to Certifiable White-Box Attacks}. The certifiable attack can be directly used as a white-box attack since it only requires hard-label query access. To explore the potential of the certifiable attack in the white-box setting, we may use a white-box localization method. Specifically, the Smoothed SSP localization method can directly compute the gradients of the noise-perturbed examples rather than leveraging the feature extractor, which may significantly improve the certified accuracy of the certifiable attack.

\vspace{0.05in}

\noindent\textbf{Targeted Certifiable Attack}. In this paper, we mainly focus on the untargeted certifiable attack. It is easy to craft a RandAE in the untargeted setting since most of the classes are adversarial classes. However, if we perform a certifiable attack by targeting specific class labels, it will be challenging to find a successful RandAE since most of the noise-perturbed input should be limited to a certain class(es). To tackle this problem, one may reduce the noise variance, which will increase the probability that most of the AEs fall into the same class. Another solution is to leverage the diffusion model to reconstruct AEs in the targeted classes.



==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Method.tex <==

\begin{figure*}[!h]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/workflow.pdf}
    \caption{Overview of crafting certified RandAE. Left: Illustration of crafting RandAE in the decision space. Right: Workflow of crafting the RandAE.}\vspace{-0.1in}
    \label{fig:framework}
\end{figure*}






% \subsection{Adversarial Success Rate Threshold}
% \label{sec: CASR}
% The certifiable attack success rate (CASR) serves as a threshold of the lower bound of ASR that the RandAE can guarantee, e.g., $90\%$. Then the task of the certifiable attack is to find the qualified RandAE with guaranteed ASR above this threshold. Specifically, 
% consider a classification problem from $\mathbb{R}^d$ to classes $\mathcal{Y}$. Given a clean input $x_o\in \mathbb{R}^d$ and its label $y\in \mathcal{Y}$. We can find an initial adversarial example $x_c$, and then craft the randomized adversarial example $x_{adv}$ by adding additional perturbations $\delta\in\mathbb{R}^d$ and noise $\epsilon\in\mathbb{R}^d$ drawn from a distribution $\mu$ to the adversarial example $x$:
% %
% \begin{equation}
%     x_{adv}=\text{Clip}\{x_c+\delta+\epsilon\}
% \end{equation}

% where $\text{Clip}\{\cdot\}$ denotes the clip operation which clips the value in each dimension of the adversarial example to a range (e.g., $[0,255]$) since RandAE may have probabilistic values out of the range.\footnote{In other domains, the RandAEs can also be bounded accordingly.} %Since the adversarial example contains a noise sampled from the distribution, we define this type of adversarial examples as ``randomized adversarial example''. 
% Any sample of the RandAE is a standard AE, and the attack success rate of the samples can be lower-bounded by a configured threshold $p$: 
% %
% % Similar to the black-box setting, the goals of the adversary are to (1) make the classification of the adversarial examples incorrect, i.e., $f(x_{adv})\neq c_o$, where $f$ denotes the classifier, and $c_o \in \mathcal{Y}$ denotes the label of input $x$; (2) make the perturbation as imperceptible as possible, i.e., $\min ||\delta||_p$, where $||\cdot||_p$ denotes the $\ell_p$-norm. The model owner's goal is to protect the model from been attacked successfully. Similar to the black-box setting, we also assume the adversary has the access to the input and polynomial-time query to the classifier's prediction.
% % However, different from traditional black-box attack, the certifiable black-box attack requires to certifiably bound the probability of successful attack.
% %
% \begin{equation}
%     \mathbb{P}(f(x_{adv})\neq y)\geq p
% \end{equation}

% where the value of constant $p$ is defined as the CASR. 

% % This means the generated adversarial examples should be guaranteed to successfully fool the classifier with at least $p$ probability. We call the probability $p$ the certifiable attack success rate (CASR), which is a pre-set threshold for certifiable attack.

% % \subsection{Certifiable Black-box Attack}

% % To provide the certifiable attack, we leverage the probabilistic methods used in randomized smoothing to design a novel mechanism for generating the adversarial attacks and certifying the attack's success rate. Specifically, we add noises to the query, derive a certified-attack region around the query samples, and shifting the certified-attack region to reduce the perturbation.

\subsection{Randomized Parallel Query}
\label{sec: batch query}
%\hl{batch}
% In the certified defense, the guarantee of robustness may rely on the probabilistic prediction of the smoothed classifier, which can be obtained by injecting the noise into the classifier. As the adversary, to guarantee the certifiable attack success rate, we also need to construct a probabilistic classifier 

% Nevertheless, from the perspective of attacks, since the adversary has the query access to the target model, the adversary can also emulate the randomization over the target model by injecting the noise into the inputs and querying the prediction results (\emph{such randomization could construct the }). %(\emph{the classifier can be considered as a randomly smoothed classifier w.r.t. the noisy queries}). 

% Our certifiable attack \hl{will} provide \emph{randomization}-based certification \cite{DBLP:conf/icml/CohenRK19}, \hl{which requires the observation of probabilistic prediction of the classifier.} \hl{In} existing probabilistic certified defense \cite{DBLP:conf/icml/CohenRK19}, the probabilistic prediction is achieved by constructing a smoothed classifier, where the model owner can inject noise into the classifier and predict the most probable class over the noise distribution. However, this remains a challenge in the certifiable black-box attack since the adversary cannot manipulate the target classifier. 

%\vspace{-0.3in}
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/Random Query Batch.pdf}
    \vspace{-0.1in}
    \caption{Illustration of Randomized Parallel Query---It returns the probability $Q(x)$ that $x+\epsilon$ is an adversarial example. }
    \label{fig:RQB}
\end{figure}

Computing the exact probability $\mathbb{P}[f(x_{adv})\neq y]$ is intractable due to the high-dimensional continuous input space. Alternatively, we estimate its low bound probability by Monte Carlo method. This requires the adversary to query the classifier with random instances sampled from an \randAE. %It is worth 
By noting that random instances can be queried efficiently in parallel, 
% Therefore, 
we propose the Randomized Parallel Query (RPQ) to compute the lower bound of the attack success probability as below:
\begin{align}
 Q(x')=\underline{p_{adv}} &\leq \mathbb{P}[f(x'+\epsilon) \neq y], \,  \epsilon \sim \varphi(0,\boldsymbol{\kappa})
%    Q(x')=\underline{p_{adv}} &\leq \mathbb{P}[f(\text{Clip}\{x'+\epsilon\}) \neq y], \,  \epsilon \sim \varphi(0,\boldsymbol{\kappa})
    % \\
    % \textit{where}~& \epsilon \sim \varphi(0,\boldsymbol{\kappa})
\end{align}
The lower bound probability $\underline{p_{adv}}$ can be estimated by Binomial testing using Clopper-Pearson confidence interval \cite{lecuyer2019certified} following the Algorithm \ref{alg:Monte Carlo}, where the $\textsc{LowerConfBound}(k,N_m,1-\alpha)$ returns the one-sided $(1-\alpha)$ lower confidence interval.%\footnote{$x'+\epsilon$ will be clipped to the valid values}. %The input values are clipped to the normal range and will not affect the lower-bound computation. For simplicity of notations, we skip $\text{Clip}\{\cdot\}$ in the notations in the rest of this work (by considering it as the default setting).

\begin{algorithm}[!h]
\small
\caption{Lower Bound of Attack Success Probability}
\label{alg:Monte Carlo}
\begin{algorithmic}[1]
\Require The noise distribution $\varphi(0, \boldsymbol{\kappa})$, mean of \randAE~ $x'$, classifier $f$, confidence level $\alpha$, Monte Carlo samples 
%sampling batch number 
$N_m$, ground truth label $y$. {\color{red} BW: where is the input example?}
\Ensure The lower bound of attack success probability $\underline{p_{adv}}$
\State $\epsilon_1, \epsilon_2,...,\epsilon_{N_m} \sim \varphi(0, \boldsymbol{\kappa})$
%\State Incorrect prediction count $k \leftarrow \sum^{i=1}_{N_m}\mathbf{1} [f(\text{Clip}\{x'+\epsilon_i\})\neq y]$
\State Incorrect prediction count $k \leftarrow \sum^{i=1}_{N_m}\mathbf{1} [f(x'+\epsilon_i)\neq y]$
\State \Return $\underline{p_{adv}} \leftarrow \textsc{LowerConfBound}(k,N_m,1-\alpha)$
\end{algorithmic}
\end{algorithm}



% To obtain the probabilistic prediction of the classifier, we propose to inject the noise into the queries given any arbitrary target model. 
% Specifically, for any input pair $(x,y)$, any target classifier $f: \mathbb{R}^d \rightarrow \mathcal{Y}$, and the noise $\epsilon$, the adversary can perform the randomized parallel query (RPQ):
% % \vspace{-0.05in}
% % 
% \begin{equation}
%     Q(x)=\mathbb{P}[f(\text{Clip}\{x+\epsilon\}) \neq y]
% \end{equation}
% % \vspace{-0.3in}

% where $Q(x)$ denotes the result of the randomized parallel query, which is the probability of the incorrect prediction in the presence of noise (see Figure \ref{fig:RQB}). This probability can be bounded by using Monte Carlo sampling and hypothesis testing, e.g., the Binomial test, which is widely adopted by certified defense methods \cite{DBLP:conf/icml/CohenRK19,zhang2020black}. Therefore, the probability is computed based on a batch of queries to the classifier, and the batch number is determined by the Monte Carlo sampling number $N_m$. %Note that, the clip operation is necessary after the noise injection since the adversarial example should follow the image formation.  
% Although the clip operation $\text{Clip}$ will truncate the noise distribution (e.g., fitting into the range of pixel values in the image domain), it will not affect the guarantee since we can construct a new classifier $f'(\cdot)\equiv f(\text{Clip}\{\cdot\})$ and certifying the attack on this new classifier $f'$ is equivalent to that on $f$. For simplicity of notations, we skip $\text{Clip}\{\cdot\}$ in the notations in the rest of this work (by considering it as the default setting). 

% % Moreover, in the certified defense, the smoothed classifier is usually trained on the noisy data to improve the classification performance on noisy data. Although in the certifiable attack, the target model is a standard classifier trained on the data without noise, high certification accuracy for certifiable attack can be easily achieved (see Section \ref{sec:Experiment} for the experimental results) since \emph{the false classes are the majority out of all the classes}.

% The certifiable attack is designed based on a batch of randomized queries that can be run in parallel. It returns the estimated probability of the wrong classes over the distribution of the RandAE. Such a batched query can boost the efficiency of the attack, given the fact that parallel computing is widely used in machine learning systems. For example, only 10-20 batches of randomized queries are sufficient to craft a RandAE with $90\%$ CASR, compared to a sequence of hundreds of queries in empirical attacks \cite{andriushchenko2020square}.

% Once the RPQ satisfies certain conditions, the RandAE can be crafted and the success of the attack can be guaranteed with provable confidence. %We will establish the theory to craft the RandAE and guarantee the attack's success in Section \ref{sec:theory}.


%Now we can query the lower bound of the attack success probability given an \randAE, but 
Next, how to find the qualified \randAE~ satisfying Eq. (\ref{eq:target}) is a core problem, known as ``Localization''. This is essentially an empirical black-box attack problem that many empirical attack algorithms can be adapted. We will introduce two different Localization methods in Section \ref{sec:initialization}. Another important problem is to minimize the perturbation size of \randAE. In the experiments, we observed that some \randAE~ are ``over-qualified'', i.e., $\underline{p_{adv}}\gg p$. This usually comes with a large perturbation size since the larger perturbation the more likely it fools the classifier. To solve this problem, we propose to reduce the perturbation size by shifting the \randAE~ while theoretically maintaining the condition Eq. (\ref{eq:target}), known as ``Shifting''. The theory of shifting is present in Section~\ref{sec:theory}.

\subsection{Certification for \randAE~ Shifting}
\label{sec:theory}
% In the certified attack, the randomized query starts from a random adversarial example $x_c+\delta$ that has a query result $Q(x_c+\delta) \geq p$. Based on the randomized query, an certified-attack region is constructed around the random adversarial example, within which the adversarial attack maintains the same attack ability. The theorem that generates the adversarial example and guarantees the attack success rate is shown in Theorem \ref{thm1}.




We propose a theory on shifting the \randAE~ while maintaining the attack success probability. 
We denote $\varphi(x'+\delta,\boldsymbol{\kappa})$ as a shifted distribution for the \randAE~ $\varphi(x', \boldsymbol{\kappa})$ by a perturbation $\delta$. 
%Specifically, the \randAE~ $\varphi(x', \boldsymbol{\kappa})$ can be shifted by a $\delta \in \mathbb{R}^d$ perturbation, denoted as $\varphi(x'+\delta,\boldsymbol{\kappa})$. 
Then the shifted \randAE~ maintains the guarantee if $\delta$ satisfies the condition presented in Theorem \ref{thm1}.

% The certification starts from finding a standard adversarial example $x_c$ such that the lower bound of the randomized parallel query is larger than the pre-configured CASR $p$, then we construct the RandAE as $x_{adv}=x_c+\delta+\epsilon$, and guarantee the attack success rate of the sampled AEs for all the perturbations $\delta$ computed by our theorem. The theory of certifying a RandAE is presented in Theorem \ref{thm1}.

\begin{thm}{(\textbf{Certifiable Adversarial Distribution Shifting})} 
%Let $f: \mathbb{R}^d \rightarrow \mathbb{R}^1$ be any deterministic or random function, 
Let $f$ be a classifier, $x_o$ be a clean input with label $y$, and 
%$y$ be the label of $x_o$. 
%Let 
$\epsilon$ be the noise drawn from any continuous probability density function  $\varphi(0,\boldsymbol{\kappa})$. Let $p$ be the pre-configured attack success possibility threshold. Denote $\underline{p_{adv}} \in [0,1]$ as the lower bound of the attack success probability. If there exists an input $x'$ such that
\begin{equation}
    \mathbb{P}[f(x'+\epsilon)\neq y]\geq \underline{p_{adv}}=Q(x')\geq p
\label{thm1 condition}
\end{equation}
then the attack success probability  $\mathbb{P}[f(x'+\delta+\epsilon)\neq y]\geq p$ is guaranteed for any shifting perturbation $\delta$ that satisfies:
\begin{equation}
    \Phi_+[\Phi_-^{-1}(\underline{p_{adv}})]\geq p
\label{thm1 condition2}
\end{equation}
where $\Phi_-^{-1}$ denotes the inverse cumulative density function (CDF) of the random variable $\frac{\varphi(\epsilon-\delta, \boldsymbol{\kappa})}{\varphi(\epsilon,\boldsymbol{\kappa})}$, and $\Phi_+$ denotes the CDF of the random variable $\frac{\varphi(\epsilon, \boldsymbol{\kappa})}{\varphi(\epsilon+\delta, \boldsymbol{\kappa})}$.

\label{thm1}
\end{thm}

\begin{proof}
See detailed proof in Appendix \ref{apd:thm1 proof}.
\end{proof} 

% \vspace{5 mm}




Theorem \ref{thm1} ensures the minimum attack success probability of $\varphi(x'+\delta,\boldsymbol{\kappa})$ if Eq. (\ref{thm1 condition}) and Eq. (\ref{thm1 condition2}) hold without querying $\varphi(x'+\delta,\boldsymbol{\kappa})$. Eq. (\ref{thm1 condition}) requires finding a $x'$ such that the randomized parallel query on samples of $\varphi(x',\boldsymbol{\kappa})$ returns a $\underline{p_{adv}}$ larger than $p$, which is the phase of Localization. Eq. (\ref{thm1 condition2}) %restricts the shifting perturbation $\delta$, ensuring 
ensures any $\delta$ meeting this condition will not reduce the attack success probability of the shifted \randAE~ below $p$. Finding a proper $\delta$ that can reduce the perturbation size of \randAE~ under this constraint is the phase of Shifting. Note that the Shifting should base on a successful Localization, i.e., $Q(x')\geq p$.
% The satisfaction of condition Eq. (\ref{thm1 condition}) is equivalent to the certification of RandAEs (once the condition Eq. (\ref{thm1 condition}) is satisfied, at least we can find $\delta=\textbf{0}$ to satisfy condition Eq. (\ref{thm1 condition2})). 

% Specifically, finding a proper $x_c$ to satisfy condition Eq. (\ref{thm1 condition}) can craft an initial successful RandAE $x_{adv}=x_c+\epsilon$. Then the condition Eq. (\ref{thm1 condition2}) extends the initial successful RandAE to a neighboring area. It creates an area of $\delta$ such that within this area, the RandAE $x_{adv}=x_c+\delta+\epsilon$ can be equally guaranteed to have at least $p$ attack success rate.
% The satisfaction of condition Eq. (\ref{thm1 condition2}) allows the adversary to further find a more optimal RandAE within this area by finding a proper $\delta$. For example, under the constraint of condition Eq. (\ref{thm1 condition2}), we can find a perturbation $\delta$ towards the clean input to reduce the perturbation. In conclusion, these two conditions formalize two important problems in crafting the RandAE: the certified RandAE localization (see Section \ref{sec:initialization}) and the certified RandAE shifting (see Section \ref{sec:shifting}).

Note that Theorem \ref{thm1} works for any continuous noise distributions, e.g., Gaussian, Laplace, Exponential, and mixture density PDFs. 
We also present the case 
%an example case of Theorem \ref{thm1} 
when the noise is Gaussian in Corollary \ref{thm2} in Appendix \ref{apd:thm2}. It shows that to ensure the ASP, the shifting perturbation $\delta$ should satisfy $||\delta||_2 \le \sigma [\Phi^{-1}(\underline{p_{adv}})-\Phi^{-1}(p)]$, where $\Phi^{-1}$ is the inverse of Gaussian CDF.

%{\color{red} BW: Curious why a smaller perturbation yields a more successful certifiable attack?}

%\hl{split this long section into two sections? Section 3: certifiable black-box attack. Section 4: Attack Design and Analysis?}

\section{Attack Design and Analysis}
\label{sec:design}

In this section, we design the certifiable attack by developing two Localization methods and one Shifting method, as well as a diffusion model-based method for further reducing the noise. Then we provide the theoretical analysis of the convergence and confidence bound of the Shifting method. 

% Specifically, we craft the RandAE by initially localizing a successful RandAE with strictly satisfied condition Eq. (\ref{thm1 condition}) (see the step \textcircled{1} in Figure \ref{fig:framework}), and then shifting the RandAE towards the clean input for reducing the perturbation size (better imperceptibility) while maintaining the guarantee (see the step \textcircled{2} in Figure \ref{fig:framework}).


\subsection{Certifiable Attack Localization}
\label{sec:initialization}

Certified attack localization aims to find an input that satisfies the condition in Eq. (\ref{thm1 condition}), which determines whether a \randAE can be certified. The simplest localization is the random localization, where the input $x$ is uniformly sampled from the input space, e.g., $[0,\ 255]^d$, followed by a \emph{randomized parallel query} to check if the $\underline{p_{adv}}$ is larger than $p$. 
% In the empirical attack, at least one adversarial example exists in the input space, so repeatedly perform the random initialization will guarantee to find an successful adversarial example. However, in the certifiable attack, the adversarial example that satisfies Eq. (\ref{thm1 condition}) may not exists. Figure \ref{} illustrate this difference between the empirical attack and certifiable attack.
However, the random localization may not generate the optimal initial adversarial examples due to the intractable stochastic process, and the perturbation may be large. Therefore, we propose two practical algorithms for Localization.

\subsubsection{Smoothed Self-supervised Localization}


To efficiently localize a better initial \randAE, we adapt the self-supervised perturbation (SSP) technique \cite{DBLP:conf/cvpr/NaseerKHKP20}. 
%to design a novel localization method for the certifiable attack, namely \emph{smoothed self-supervised perturbation} (SSSP). 
Specifically, SSP generates generic adversarial examples by distorting the low-level features extracted by a pre-trained feature extractor 
%(Multi-layers of ResNet34 pre-trained on ImageNet \cite{ILSVRC15}) 
in a self-supervised manner. Since the certifiable attack uses the Randomized Parallel Query, we compute the feature distortion over a set of random samples from \randAE. %all the samples in the batch. Therefore, we alternatively craft the adversarial example that distorts the features extracted from all the noise-perturbed inputs. Specifically, The Smoothed SSP localization returns the initial adversarial example $x_c=x_o+\delta$ such that:
%
\begin{align}
    x'= \arg \max_{x'} ~ &\mathbb{E}_{\epsilon \sim \varphi(0,\boldsymbol{\kappa})}[\| \mathcal{F}(x' +\epsilon) -\mathcal{F}(x_o+\epsilon) \|_2]\\
    & s.t. \|x'-x\|_\infty\leq \pi 
\end{align}

where $\mathcal{F}$ is a pre-trained feature extractor, $x_o$ is the clean image, $\pi$ is the perturbation budget, and $||\cdot||_p$ is the $\ell_p$-norm distance. The feature extractor is pre-trained on large-scale datasets and the low-level features can be transferred to other classifiers. Then, the proposed Smoothed SSP localization can be generalized to various classifiers to efficiently find the initial \randAE. 

To solve this optimization problem, we leverage the Projected Gradient Descent method \cite{DBLP:conf/iclr/MadryMSTV18} to update the \randAE~ in an offline manner. Let the adversarial loss be $\mathcal{L}(x')\equiv \mathbb{E}_{\epsilon \sim \varphi}[\|\mathcal{F}(x'+\epsilon)-\mathcal{F}(x_o+\epsilon)\|_2]$. Then, the \randAE can be localized by iteratively perturbing it along the direction of the gradient ascending:
%
\begin{equation}
    x'_{t+1}=x'_{t}+\eta\ sgn(\nabla_{x'_t} \mathcal{L})
\end{equation}
where $x'_t$ and $x'_{t+1}$ respectively denote the center of the current and updated initial \randAE, %$x_{c}^{t+1}$ denotes the updated center of the initial RandAE, 
$sgn(\cdot)$ is the sign function, and $\eta$ denotes the step size.
%for updating the RandAE. 

To find the initial random adversarial example (\randAE) within a small perturbation range, we adjust the perturbation budget ($\pi$) incrementally from a smaller to a larger value. The details for localizing the \randAE are summarized in Algorithm \ref{alg:initialization} and \ref{alg:sssp}. 
% The comparison of the random localization and the Smoothed SSP localization can be found in Section \ref{sec:ablation}.

\begin{algorithm}[!h]
\small
\caption{Smoothed SSP Certifiable Attack Localization}
\label{alg:initialization}
\begin{algorithmic}[1]
\Require Clean input $x_o$, feature extractor $\mathcal{F}(\cdot)$, RPQ function $Q(\cdot)$,  smoothed SSP algorithm $SSSP(\cdot)$ (Algorithm \ref{alg:sssp}), initial perturbation budget $\pi_{init}$,  %perturbation size increasing 
step size $\gamma$, ASP Threshold $p$, and maximum iterations $N_{max}$.
%, and noise distribution $\mu$.
\Ensure Mean of initial \randAE~ $x'$, number of RPQs $q$.
\State $x'=x_o$, $\pi=\pi_{init}$, $N=0$, $q=0$
\While {$Q(x')<p$ and $N<N_{max}$}
\State $N\leftarrow N+1$, $q\leftarrow q+1$, $\pi \leftarrow \pi+\gamma$
\State $x'\leftarrow SSSP(x',\ \mathcal{F},\ \pi)$
\EndWhile
\If{$Q(x')<p$}
\State \Return \textbf{Abstain}
\Else
\State \Return $x'$ and $q$ 
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!h]
\small
\caption{Smoothed Self-supervised Perturbation (SSSP)}
\label{alg:sssp}
\begin{algorithmic}[1]
\Require Mean of \randAE~ $x'$, clean input $x_o$, feature extractor $\mathcal{F}$, 
%the loss function $\mathcal{L}$, 
noise distribution $\varphi(0,\boldsymbol{\kappa})$, maximum iterations $n_{max}$,  perturbation budget $\pi$, step size $\eta$, and noise sampling number $N_s$.
\Ensure Updated mean of \randAE~ $x'$
\For {$n=1$ to $n_{max}$ }
\State $\mathcal{L}(x')\leftarrow \frac{1}{N_s}\sum_i^{N_s}[||\mathcal{F}(x'+\epsilon_i)-\mathcal{F}(x_o+\epsilon_i)||_2], \ \epsilon_i \sim \varphi$
\State $x' \leftarrow  \eta\ sgn(\nabla_{x'}\mathcal{L})$
\State $x' \leftarrow Clip(x',\ x_o-\pi,\ x_o+\pi)$
\State $x' \leftarrow Clip(x',\ 0.0,\ 1.0)$
\EndFor
\State \Return $x'$
\end{algorithmic}
\end{algorithm}

\subsubsection{Binary search Localization}

Another localization method is to randomly initialize an \randAE~ with $\underline{p_{adv}}\geq p$, then reduce the gap between $\underline{p_{adv}}$ and $p$, as well as the perturbation by binary search. The algorithm is presented in Algorithm \ref{alg:bin search}. This method is efficient in reducing the perturbation size once the initial \randAE~ is found by random search.

\begin{algorithm}[!h]
\small
\caption{Binary search Certifiable Attack Localization}
\label{alg:bin search}
\begin{algorithmic}[1]
\Require Clean input $x_o$, RPQ function $Q(\cdot)$, ASP Threshold $p$, random search iterations $N_r$, and binary search iteration $N_b$.
%, and noise distribution $\mu$.
\Ensure Mean of initial \randAE~ $x'$, number of RPQs $q$.
\State $n=0$, $m=0$, $q=0$, $x=x_o$
\While{$Q(x')<p$ and $n<N_r$}
\State $x' \sim \text{Uniform}([0,1]^d)$
\State $q\leftarrow q+1$, 
\EndWhile
\While{$m<N_b$}
\If{$Q(\frac{x+x'}{2})\geq p$}
\State $x'=\frac{x+x'}{2}$
\Else
\State $x=\frac{x+x'}{2}$
\EndIf
\EndWhile
\State \Return $x'$
\end{algorithmic}
\end{algorithm}

\setlength{\textfloatsep}{2mm}


\subsection{Certified Attack Shifting}
\label{sec:shifting}



The certifiable attack shifting aims to reduce the perturbation size of \randAE~ while maintaining the ASP guarantee for the \randAE. The localization crafts an initial \randAE, but the imperceptibility is still not optimal. In the classification, the optimal imperceptibility can be achieved when the adversarial example is close to the decision boundary. Therefore, we shift the \randAE~ towards the clean input to reduce the size of the perturbation until intersecting the decision boundary ($\underline{p_{adv}}=p$), namely ``certified attack shifting''. 


Note that the \randAE~ can be shifted by any $\delta$ satisfying Eq. (\ref{thm1 condition2}), we can shift it toward the clean input with the maximum $\delta$ that does not break the guarantee. By iteratively executing the RPQ and applying the Theorem \ref{thm1}, the \randAE~ can be repeatedly shifted with a guarantee until it approaches the decision boundary ($\underline{p_{adv}}=p$). As Corollary \ref{corollary:shifting} states, the mean of the previous \randAE~ naturally satisfies the condition of Eq. (\ref{thm1 condition}). Then, the \randAE~ can be shifted using the Theorem \ref{thm1}. This process can be repeated until $\underline{p_{adv}}=p$. Per the Corollary \ref{corollary:shifting}, although we know that $Q(x'+\delta)\geq p$, we still need to run the RPQ to update the lower bound $\underline{p_{adv}}$ for deriving the new $\delta$. 

\begin{corollary}[Certified Attack Shifting]
If a \randAE $\varphi(x'+\delta,\boldsymbol{\kappa})$ is certified, then the mean $x'+\delta$ also satisfies Condition Eq. (\ref{thm1 condition}).
\label{corollary:shifting}
\end{corollary}
\begin{proof}
If a \randAE~ is certified, then per Theorem \ref{thm1}, the ASP of $x'+\delta$ is at least $p$. Thus, let $x''=x'+\delta$, we have $\mathbb{P}[f(x''+\epsilon)\neq y)]\geq Q(x'')\geq p$, $x''$ satisfies Condition Eq. (\ref{thm1 condition}). 
\end{proof}

Now we propose to shift \randAE~ to reduce the perturbation size without affecting the provable guarantee. This problem can be solved by two steps: \emph{first finding the shifting direction, and then deriving the shifting distance while maintaining the guarantee}. Here, we design a novel shifting method to find the locally optimal \randAE~ by considering the geometric relationship between the decision boundary and the \randAE, which is called ``Geometrical Shifting''. Specifically, through using the noisy samples of \randAE~ to ``probe'' the decision boundary, we shift the RandAE~ along the decision boundary and towards the clean input until finding the local optimal point on the decision boundary (see Figure \ref{fig:shifting method} for the illustration). If none of the noisy samples can approach the decision boundary, we simply shift the \randAE~ directly toward the clean input without considering the decision boundary.  

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figs/Geometrically_shifting.pdf}
%     \caption{Geometrically shifting}
%     \label{fig:geo_shifting}
% \end{figure}

Specifically, the geometrical relationship is presented on the right-hand side of Figure \ref{fig:shifting method}.  Denote $x'$ as the mean of the current \randAE. When sampling the adversarial examples from the \randAE, we mark the failed adversarial examples as $x^1_+, x^2_+,...,x^i_+, ..., x^k_+$, aka., ``samples fell into the original class''. The normalized vector from $x_+^i$ to $x'$ is denoted as $v^i$. The normalized vector from $x'$ to $x_o$ is denoted as $u$. If the \randAE~ has no samples crossing the decision boundary, then we can shift the \randAE~ straight toward the clean input (along the direction of $u$) until it intersects the decision boundary, otherwise, the shifting should be along the decision boundary but not cross it
(without changing the certifiable attack guarantee). Note that the input space is high-dimensional, thus there could be many directions along the decision boundary. To reduce the perturbation size, the direction should be similar to the vector $u$ as much as possible. Based on these geometric analyses, the goals of the geometrical shifting can be summarized as: \emph{The shifting direction should lie relatively parallel to the direction of $u$; and be relatively vertical to the vectors $v^i$.}


 \begin{figure}[!t]
\vspace{-0.2in}
    \centering
    \includegraphics[width=\linewidth]{figs/shifting_illustration.pdf}
    \vspace{-0.15in}
    \caption{Illustration of Geometrically Shifting}
    \vspace{-0.05in}
    \label{fig:shifting method}
\end{figure}



Formally, denoting the shifting direction as $w$, 
%if we use the cosine similarity to measure the direction similarity, 
then the goal of finding the shifting direction can be formulated as:
%\vspace{-0.15in}
\begin{equation}
    w =\arg \max \sum_{i=1}^k \sin(v^i,w) + \cos(u,w)
\label{eq:geo eq}
\end{equation}
where $\sin(\cdot)$ and $\cos(\cdot)$ denote the sine and cosine function similarity of two vectors, 
respectively. Eq. (\ref{eq:geo eq}) can be solved via the gradient ascent algorithm. 

%Hence, the shifting direction can be found by solving Eq. (\ref{eq:geo eq}) and 
Next, the shifting distance can be determined by finding the maximum $||\delta||_2$ that satisfies the constraint of Eq. (\ref{thm1 condition2}). Specifically, the maximum $||\delta||_2$ is achieved when the equality in Eq. (\ref{thm1 condition2}) holds. We use binary search to approach the equality and use the Monte Carlo method to estimate the CDF of random variable $\frac{\varphi(\epsilon-\delta, \boldsymbol{\kappa})}{\varphi(\epsilon, \boldsymbol{\kappa})}$ and $\frac{\varphi(\epsilon, \boldsymbol{\kappa})}{\varphi(\epsilon+\delta, \boldsymbol{\kappa})}$, similar to \cite{hong2022unicr}. Algorithm \ref{alg:shifting direction} and \ref{alg:shifting distance} show the details on finding the shifting direction and distance, respectively.

\vspace{0.05in}

\noindent\textbf{Convergence Analysis and Confidence Bound:}
Note that any $\delta$ computed by the Algorithm \ref{alg:shifting distance} will not violate the certifiable attack guarantee since it strictly ensures $\Phi_+[\Phi^{-1}_-(\underline{p_{adv}})] \ge p$, even when the shifting direction is not parallel to the decision boundary.
We analyze the convergence of the algorithms and the confidence bound. \emph{With the centralized noise distribution, the shifting algorithm is guaranteed to converge once the initial \randAE is localized.}
% We show this theoretical guarantee in Proposition \ref{prop:bound}.

\begin{proposition}
\label{prop:bound}
If the noise distribution $\mu(x)$ decreases as the $|x|$ increases, with the satisfaction of Eq. (\ref{thm1 condition}), given any vector direction $w$, the Shifting Distance algorithm is guaranteed to find the $\delta$ such that $\Phi_+[\Phi_-^{-1}(\underline{p_{adv}})]= p$ with confidence $(1-\alpha_o)(1-2e^{-2N_m\Delta^2})^2$, where $(1-\alpha_o)$ is the confidence for the $\underline{p_{adv}}$ estimation, $N_m$ is the Monte Carlo sampling number, and $\Delta$ is the error bound for the CDF estimation.
\end{proposition}

\begin{proof}
See detailed proof in Appendix \ref{apd:theoretical bound}.
\end{proof}

\begin{algorithm}[!t]
\small
\caption{Shifting Direction}
\label{alg:shifting direction}
\begin{algorithmic}[1]
\Require Mean of the \randAE~ $x'$, clean input $x_o$,  vectors $\{v^i\}$, a vector $u$, maximum iteration $M$, updating step size $\eta'$.
\Ensure The shifting direction $w$
\State Initialize $w$ with random noise
\If{ $\{v^i\}$ is empty}
\State $w=x_o-x'$
\Else
\For {$j=1$ to $M$}
\State $w\leftarrow w+\eta'\ sgn[\nabla_w({\sum_{i=1}^k \sin(v^i,w) + \cos(u,w)})]$
\State $w\leftarrow \frac{w}{||w||_2}$
\EndFor
\EndIf
\State \Return $w$
\end{algorithmic}
\end{algorithm}


\setlength{\textfloatsep}{2mm}


\begin{algorithm}[!t]
\small
\caption{Shifting Distance}
\label{alg:shifting distance}
\begin{algorithmic}[1]
\Require Mean of \randAE~ $x'$,  noise distribution $\varphi$, Monte Carlo sampling number $N_m$,  confidence $1-\alpha_o$, randomized query function $Q(\cdot)$, the shifting direction algorithm $SD(\cdot)$ (Algorithm \ref{alg:shifting direction}), error threshold $e$, ASP Threshold $p$.
\Ensure The shifting perturbation $\delta$
\State $w \leftarrow SD(x')$
\State $\underline{p_{adv}} \leftarrow Q(x', 1-\alpha_o, N_m)$
\State find a scalar $a$ such that $\delta=a w$ and $ \Phi_+[\Phi_-^{-1}(\underline{p_{adv}})] > p$
\State find a scalar $b$ such that $\delta=b w$ and $ \Phi_+[\Phi_-^{-1}(\underline{p_{adv}})] < p$
% \State $\delta=\frac{(a+b)}{2}w$
\While {$\Phi_+[\Phi_-^{-1}(\underline{p_{adv}})]<p$ or $ > p+e$}
\If {$\Phi_+[\Phi_-^{-1}(\underline{p_{adv}})] >p$}
\State $a\leftarrow \frac{(a+b)}{2}$
\Else
\State $b\leftarrow \frac{(a+b)}{2}$
\EndIf
\State $\delta\leftarrow \frac{(a+b)}{2}w$
\EndWhile
\State \Return $\delta$
\end{algorithmic}
\end{algorithm}


\setlength{\textfloatsep}{2mm}



\subsection{Imperceptibility with Diffusion Models}
{\color{red} BW: This parts seems just a plus. Better put into appendix to make the paper concise.}

The certifiable adversarial examples sampled from \randAE~ are noise-injected inputs that might be perceptible when the noise is large. Here, we leverage the recent innovation for image synthesis, i.e., diffusion model \cite{ho2020denoising}, to denoise the certifiable adversarial examples for better imperceptibility. The key idea is to consider the noise-perturbed adversarial examples as the middle sample in the forward process of diffusion models \cite{carlini2022certified,zhang2023diffsmooth}. This improves the imperceptibility and the diversity of the adversarial examples.

Specifically, the closed-form sampling in the forward process at timestep $t$ in \cite{ho2020denoising} can be written as:
%
\begin{equation}
\label{eq:diffusion}
    x_t=\sqrt{\overline{\alpha}_t}x_0+\sqrt{1-\overline{\alpha}_t}\epsilon_0
\end{equation}
where $\overline{\alpha}_t$ is the parameter that indicates the transformation of the image in the forward process, $x_0$ is the clean image, and $\epsilon_0$ is a noise drawn from the standard normal distribution $\mathcal{N}(0,1)$. The certifiable adversarial examples when adding noise $\epsilon_0$ can be expressed as:
\begin{equation}
    x_{adv}=x'+\delta+\epsilon_0
\end{equation}
%where the noise $\epsilon_0$ is drawn from the standard normalized distribution. 
We can consider the certifiable adversarial example $x_{adv}$ as the sample $x_t$ in Eq. (\ref{eq:diffusion}) by transforming $x_{adv}$ to $\sqrt{\overline{\alpha}_t}x_{adv}$ and satisfying these conditions: (1) $x'+\delta=x_0$ and (2) 
    $\sqrt{\overline{\alpha}_t}\sigma=\sqrt{1-\overline{\alpha}_t}$. Then, we have  
    $\overline{\alpha}_t=\frac{1}{\sigma^2+1}$ to bridge diffusion model and the certifiable attack.

By finding the corresponding time step $t$ and parameter $\overline{\alpha_t}$, we can leverag the reverse process $\mathcal{R}(\cdot)$ of the diffusion model to denoise the $x_{adv}$:
\begin{equation}
    x_{adv}'=\mathcal{R}(\mathcal{R}(...\mathcal{R}(\sqrt{\overline{\alpha}_t}x_{adv})))
\end{equation}

Note that the reverse denoising process can be integrated into our attack framework immediately by simply replacing $x_{adv}$ with $x_{adv}'$ in all processes. It will not affect the guarantee since we can consider the denoise transformation as a part of the classification, i.e., constructing a new target model $f'(x_{adv})=f(\mathcal{R}(\mathcal{R}(...\mathcal{R}(\sqrt{\overline{\alpha_t}} x_{adv}))))$ given any $f$. 
% We will evaluate how denoising improves the imperceptibility of certifiable adversarial examples in Section \ref{sec:exp diffusion}.








==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> exp_audio.tex <==


\subsection{Setup}



\subsection{Results}


\begin{table}[!h]
%\small
  \caption{Performance of Certifiable Black-box Attack with Gaussian Noise. The CASR threshold is set as $p=90\%$, and the $\sigma$ denotes the standard deviation of the noise. (smt ssp)}
    \centering
    \begin{tabular}{c|c| c c c c}
    \hline
    \hline
         & $\sigma$ & $Pert_{sample}$ &$Pert_{center}$ & RQB & Certified Acc.  \\
    \hline
         \multirow{4}*{\rotatebox{90}{\footnotesize \ \ \ Audio}} 
& 0.05 & 18.35 & 12.67 & 5.42 & 100\% \\
& 0.1 & 26.71 & 12.70 & 3.72 & 100\% \\
& 0.15 & 35.82 & 12.63 & 3.12 & 100\% \\
    \hline
    \hline
    \end{tabular}
    \label{tab:diff_variance_audio}
\end{table}

\begin{table}[!h]
%\small
  \caption{Performance of Certifiable Black-box Attack with Gaussian Noise. The CASR threshold is set as $p=90\%$, and the $\sigma$ denotes the standard deviation of the noise. (random)}
    \centering
    \begin{tabular}{c|c| c c c c}
    \hline
    \hline
         & $\sigma$ & $Pert_{sample}$ &$Pert_{center}$ & RQB & Certified Acc.  \\
    \hline
         \multirow{4}*{\rotatebox{90}{\footnotesize \ \ \ Audio}} 
& 0.05 & 161.43 & 161.03 & 74.00 & 100\% \\
& 0.1 & 159.21 & 157.53 & 73.88 & 100\% \\
& 0.15 & 157.78 & 154.00 & 73.86 & 100\% \\
    \hline
    \hline
    \end{tabular}
    \label{tab:diff_variance_audio_random}
\end{table}


\begin{table}[!h]
%\small
  \caption{Performance of Certifiable Black-box Attack with Gaussian noise and standard deviation $\sigma=0.1$.}
    \centering
    \begin{tabular}{c|c|c c c c}
    \hline
    \hline
 & p & $Pert_{sample}$ &$Pert_{center}$ & RQB & Certified Acc.  \\ 
        \hline
             \multirow{6}{*}[-1mm]{\rotatebox{90}{Audio}} 
& 50\% & 26.64 & 12.55 & 5.31 & 100\% \\
& 60\% & 26.65 & 12.57 & 5.08 & 100\% \\
& 70\% & 26.66 & 12.60 & 4.87 & 100\% \\
& 80\% & 26.68 & 12.63 & 4.49 & 100\% \\
& 90\% & 26.71 & 12.70 & 3.72 & 100\% \\
& 95\% & 26.74 & 12.78 & 3.05 & 100\% \\
                                                     
    \hline
    \hline
    \end{tabular}
  
    \label{tab:diff_p_audio}
\end{table}



\begin{table*}[!h]
    \centering
    % \setlength\tabcolsep{3pt}
        \caption{Ablation Study with CASR threshold $p=90\%$. The noise distribution is Gaussian noise with $\sigma=0.25$. Audio}
   % \small
    \begin{tabular}{c|c|c|c|c c c c}
    \hline
    \hline
        & Method & Initialization & Shifting  & $Pert_{sample}$ &$Pert_{center}$ & RQB & Certified Acc.\\
    \hline
        \multirow{4}{*}[-0mm]{\rotatebox{90}{Audio}} 
        & Baseline A & random  & no shifting     &  &  &  & 100\% \\
        & Baseline B & random  & geo. shifting   & 159.21 & 157.53 & 73.88 & 100\% \\
        & Baseline C & SSSP    & no shifting     & 26.70 & 12.71 & 4.20 & 100\% \\
        & Baseline D & SSSP    & geo. shifting   & 26.71 & 12.70 & 3.72 & 100\% \\
    \hline
    \hline
    \end{tabular}
    \label{tab:ablation_study_audio}
\end{table*}





==> tables/CIFAR10_AT_resnet_l2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Attack performance under TRADES Adversarial Training ($\ell_2$ perturbation) on ResNet and CIFAR10}
\label{tab:AT_cifar10_resnet_l2}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lccccc}
\hline
Attack &
  \begin{tabular}[c]{@{}c@{}}Query\\ Type\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Perturbation\\ Type\end{tabular} &
  Query &
  Model Acc &
  Distance \\ \hline
\multicolumn{1}{l|}{Bandit}    & Score & \multicolumn{1}{c|}{$\ell_2$}     & 860  & 1.5  & 2.44 \\
\multicolumn{1}{l|}{NES}       & Score & \multicolumn{1}{c|}{$\ell_2$}     & 3535 & 9.5  & 0.99 \\
\multicolumn{1}{l|}{Simple}    & Score & \multicolumn{1}{c|}{$\ell_2$}     & 4062 & 2.1  & 1.29 \\
\multicolumn{1}{l|}{Square}    & Score & \multicolumn{1}{c|}{$\ell_2$}     & 991  & 4.6  & 2.95 \\
\multicolumn{1}{l|}{ZOSignSGD} & Score & \multicolumn{1}{c|}{$\ell_2$}     & 3505 & 15.1 & 0.77 \\
\multicolumn{1}{l|}{Boundary}  & Label & \multicolumn{1}{c|}{$\ell_2$}     & 771  & 40.7 & 1.19 \\
\multicolumn{1}{l|}{GeoDA}     & Label & \multicolumn{1}{c|}{$\ell_2$}     & 1506 & 14.3 & 2.85 \\
\multicolumn{1}{l|}{HSJ}       & Label & \multicolumn{1}{c|}{$\ell_2$}     & 1332 & 5.1  & 3.53 \\
\multicolumn{1}{l|}{Opt}       & Label & \multicolumn{1}{c|}{$\ell_2$}     & 2890 & 41.6 & 2.39 \\
\multicolumn{1}{l|}{SignOPT}   & Label & \multicolumn{1}{c|}{$\ell_2$}     & 1766 & 33.6 & 2.76 \\
\multicolumn{1}{l|}{PointWise} & Label & \multicolumn{1}{c|}{unrestricted} & 4845 & 0.6  & 5.36 \\
\multicolumn{1}{l|}{SparseEvo} & Label & \multicolumn{1}{c|}{unrestricted} & 9697 & 0.4  & 6.03 \\ \hline
\multicolumn{1}{l|}{\textbf{CA(sssp)}} &
  Label &
  \multicolumn{1}{c|}{unrestricted} &
  809 &
  20.4 &
  6.06 \\
\multicolumn{1}{l|}{\textbf{CA(bin search)}} &
  Label &
  \multicolumn{1}{c|}{unrestricted} &
  461 &
  0.0 &
  8.18 \\ \hline
\end{tabular}%
}
\end{table}

==> tables/CIFAR10_AT_resnet_linf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Attack performance under TRADES Adversarial Training ($\ell_\infty$ perturbation) on ResNet and CIFAR10}
\label{tab:AT_cifar10_resnet_linf}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lccccc}
\hline
Attack &
  \begin{tabular}[c]{@{}c@{}}Query\\ Type\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Perturbation\\ Type\end{tabular} &
  Query &
  Model Acc &
  Distance \\ \hline
\multicolumn{1}{l|}{Bandit}       & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 1601 & 10.2 & 4.32 \\
\multicolumn{1}{l|}{NES}          & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 1474 & 27.4 & 2.27 \\
\multicolumn{1}{l|}{Parsimonious} & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 630  & 5.3  & 4.35 \\
\multicolumn{1}{l|}{Sign}         & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 439  & 4.4  & 4.37 \\
\multicolumn{1}{l|}{Square}       & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 854  & 5.7  & 4.39 \\
\multicolumn{1}{l|}{ZOSignSGD}    & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 1196 & 37.0 & 2.21 \\
\multicolumn{1}{l|}{GeoDA}        & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 1358 & 41.9 & 1.99 \\
\multicolumn{1}{l|}{HSJ}          & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 2149 & 36.5 & 1.92 \\
\multicolumn{1}{l|}{Opt}          & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 1871 & 73.0 & 0.19 \\
\multicolumn{1}{l|}{RayS}         & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 721  & 7.3  & 4.29 \\
\multicolumn{1}{l|}{SignFlip}     & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 2240 & 24.4 & 3.36 \\
\multicolumn{1}{l|}{SignOPT}      & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 832  & 69.3 & 0.15 \\
\multicolumn{1}{l|}{PointWise}    & Label & \multicolumn{1}{c|}{unrestricted}  & 3460 & 9.3  & 4.38 \\
\multicolumn{1}{l|}{SparseEvo}    & Label & \multicolumn{1}{c|}{unrestricted}  & 8691 & 9.1  & 5.10 \\ \hline
\multicolumn{1}{l|}{\textbf{CA(sssp)}} &
  Label &
  \multicolumn{1}{c|}{unrestricted} &
  548 &
  21.2 &
  4.29 \\
\multicolumn{1}{l|}{\textbf{CA(bin search)}} &
  Label &
  \multicolumn{1}{c|}{unrestricted} &
  412 &
  9.8 &
  6.31 \\ \hline
\end{tabular}%
}
\end{table}

==> tables/ImageNet_post_RAND_vgg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Attack performance under RAND Post-processing Defense on VGG and ImageNet}
\label{tab:imagenet_post_RAND_vgg}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lccccc}
\hline
Attack &
  \begin{tabular}[c]{@{}c@{}}Query\\ Type\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Perturbation\\ Type\end{tabular} &
  Query &
  Model Acc &
  Distance \\ \hline
\multicolumn{1}{l|}{Bandit}    & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 8   & 1.6  & 26.65 \\
\multicolumn{1}{l|}{NES}       & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 340 & 11.0 & 8.96  \\
\multicolumn{1}{l|}{Parsimonious} &
  Score &
  \multicolumn{1}{c|}{$\ell_\infty$} &
  310 &
  48.5 &
  26.32 \\
\multicolumn{1}{l|}{Sign}      & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 121 & 7.6  & 26.39 \\
\multicolumn{1}{l|}{Square}    & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 7   & 0.2  & 26.66 \\
\multicolumn{1}{l|}{ZOSignSGD} & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 344 & 14.7 & 9.22  \\
\multicolumn{1}{l|}{GeoDA}     & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 130 & 38.4 & 17.25 \\
\multicolumn{1}{l|}{HSJ}       & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 204 & 52.8 & 10.48 \\
\multicolumn{1}{l|}{Opt}       & Label & \multicolumn{1}{c|}{$\ell_\infty$} & --  & --   & --    \\
\multicolumn{1}{l|}{RayS}      & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 262 & 43.7 & 28.40 \\
\multicolumn{1}{l|}{SignFlip}  & Label & \multicolumn{1}{c|}{$\ell_\infty$} & --  & --   & --    \\
\multicolumn{1}{l|}{SignOPT}   & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 445 & 64.5 & 0.78  \\
\multicolumn{1}{l|}{Bandit}    & Score & \multicolumn{1}{c|}{$\ell_2$}      & 557 & 4.1  & 13.25 \\
\multicolumn{1}{l|}{NES}       & Score & \multicolumn{1}{c|}{$\ell_2$}      & --  & --   & --    \\
\multicolumn{1}{l|}{Simple}    & Score & \multicolumn{1}{c|}{$\ell_2$}      & --  & --   & --    \\
\multicolumn{1}{l|}{Square}    & Score & \multicolumn{1}{c|}{$\ell_2$}      & 29  & 0.4  & 27.48 \\
\multicolumn{1}{l|}{ZOSignSGD} & Score & \multicolumn{1}{c|}{$\ell_2$}      & --  & --   & --    \\
\multicolumn{1}{l|}{Boundary}  & Label & \multicolumn{1}{c|}{$\ell_2$}      & --  & --   & --    \\
\multicolumn{1}{l|}{GeoDA}     & Label & \multicolumn{1}{c|}{$\ell_2$}      & 135 & 40.8 & 17.26 \\
\multicolumn{1}{l|}{HSJ}       & Label & \multicolumn{1}{c|}{$\ell_2$}      & 219 & 48.4 & 18.20 \\
\multicolumn{1}{l|}{Opt}       & Label & \multicolumn{1}{c|}{$\ell_2$}      & --  & --   & --    \\
\multicolumn{1}{l|}{SignOPT}   & Label & \multicolumn{1}{c|}{$\ell_2$}      & 405 & 42.8 & 18.77 \\
\multicolumn{1}{l|}{PointWise} & Label & \multicolumn{1}{c|}{unrestricted}  & --  & --   & --    \\
\multicolumn{1}{l|}{SparseEvo} & Label & \multicolumn{1}{c|}{unrestricted}  & --  & --   & --    \\ \hline
\multicolumn{1}{l|}{\textbf{CA(sssp)}} &
  Label &
  \multicolumn{1}{c|}{unrestricted} &
  194 &
  2.4 &
  15.50 \\
\multicolumn{1}{l|}{\textbf{CA(bin search)}} &
  Label &
  \multicolumn{1}{c|}{unrestricted} &
  603 &
  0.0 &
  29.85 \\ \hline
\end{tabular}%
}
\end{table}

==> tables/Imagenet_RAND_vgg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Attack performance under RAND Pre-processing Defense on VGG and ImageNet}
\label{tab:imagenet_RAND_vgg}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lccccc}
\hline
Attack &
  \begin{tabular}[c]{@{}c@{}}Query\\ Type\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Perturbation\\ Type\end{tabular} &
  Query &
  Model Acc &
  Distance \\ \hline
\multicolumn{1}{l|}{Bandit}       & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 9   & 5.1  & 25.78 \\
\multicolumn{1}{l|}{NES}          & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 432 & 51.0 & 10.31 \\
\multicolumn{1}{l|}{Parsimonious} & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 218 & 65.0 & 25.53 \\
\multicolumn{1}{l|}{Sign}         & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 115 & 44.4 & 25.47 \\
\multicolumn{1}{l|}{Square}       & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 5   & 5.8  & 26.20 \\
\multicolumn{1}{l|}{ZOSignSGD}    & Score & \multicolumn{1}{c|}{$\ell_\infty$} & 457 & 52.9 & 10.40 \\
\multicolumn{1}{l|}{GeoDA}        & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 132 & 42.0 & 18.22 \\
\multicolumn{1}{l|}{HSJ}          & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 202 & 55.4 & 11.24 \\
\multicolumn{1}{l|}{Opt}          & Label & \multicolumn{1}{c|}{$\ell_\infty$} & --  & --   & --    \\
\multicolumn{1}{l|}{RayS}         & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 249 & 51.4 & 28.94 \\
\multicolumn{1}{l|}{SignFlip}     & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 43  & 54.1 & 16.91 \\
\multicolumn{1}{l|}{SignOPT}      & Label & \multicolumn{1}{c|}{$\ell_\infty$} & 382 & 70.9 & 0.35  \\
\multicolumn{1}{l|}{Bandit}       & Score & \multicolumn{1}{c|}{$\ell_2$}      & 535 & 61.0 & 11.82 \\
\multicolumn{1}{l|}{NES}          & Score & \multicolumn{1}{c|}{$\ell_2$}      & 275 & 67.4 & 0.43  \\
\multicolumn{1}{l|}{Simple}       & Score & \multicolumn{1}{c|}{$\ell_2$}      & --  & --   & --    \\
\multicolumn{1}{l|}{Square}       & Score & \multicolumn{1}{c|}{$\ell_2$}      & 41  & 18.7 & 26.83 \\
\multicolumn{1}{l|}{ZOSignSGD}    & Score & \multicolumn{1}{c|}{$\ell_2$}      & 245 & 69.0 & 0.29  \\
\multicolumn{1}{l|}{Boundary}     & Label & \multicolumn{1}{c|}{$\ell_2$}      & 42  & 44.6 & 19.60 \\
\multicolumn{1}{l|}{GeoDA}        & Label & \multicolumn{1}{c|}{$\ell_2$}      & 138 & 48.3 & 17.03 \\
\multicolumn{1}{l|}{HSJ}          & Label & \multicolumn{1}{c|}{$\ell_2$}      & 215 & 51.1 & 18.66 \\
\multicolumn{1}{l|}{Opt}          & Label & \multicolumn{1}{c|}{$\ell_2$}      & --  & --   & --    \\
\multicolumn{1}{l|}{SignOPT}      & Label & \multicolumn{1}{c|}{$\ell_2$}      & 386 & 53.4 & 18.42 \\
\multicolumn{1}{l|}{PointWise}    & Label & \multicolumn{1}{c|}{unrestricted}  & 937 & 56.5 & 12.64 \\
\multicolumn{1}{l|}{SparseEvo}    & Label & \multicolumn{1}{c|}{unrestricted}  & --  & --   & --    \\ \hline
\multicolumn{1}{l|}{\textbf{CA(sssp)}} &
  Label &
  \multicolumn{1}{c|}{unrestricted} &
  203 &
  2.2 &
  15.90 \\
\multicolumn{1}{l|}{\textbf{CA(bin search)}} &
  Label &
  \multicolumn{1}{c|}{unrestricted} &
  603 &
  0.0 &
  29.24 \\ \hline
\end{tabular}%
}
\end{table}
